Vision Mamba in Remote Sensing: A Comprehensive Survey of Techniques, Applications and Outlook

Deep learning has profoundly transformed remote sensing, yet prevailing architectures like Convolutional Neural Networks (CNNs) and Vision Transformers (ViTs) remain constrained by critical trade-offs: CNNs suffer from limited receptive fields, while ViTs grapple with quadratic computational complexity, hindering their scalability for high-resolution remote sensing data. State Space Models (SSMs), particularly the recently proposed Mamba architecture, have emerged as a paradigm-shifting solution, combining linear computational scaling with global context modeling. This survey presents a comprehensive review of Mamba-based methodologies in remote sensing, systematically analyzing about 120 Mamba-based remote sensing studies to construct a holistic taxonomy of innovations and applications. Our contributions are structured across five dimensions: (i) foundational principles of vision Mamba architectures, (ii) micro-architectural advancements such as adaptive scan strategies and hybrid SSM formulations, (iii) macro-architectural integrations, including CNN-Transformer-Mamba hybrids and frequency-domain adaptations, (iv) rigorous benchmarking against state-of-the-art methods in multiple application tasks, such as object detection, semantic segmentation, change detection, etc. and (v) critical analysis of unresolved challenges with actionable future directions. By bridging the gap between SSM theory and remote sensing practice, this survey establishes Mamba as a transformative framework for remote sensing analysis. To our knowledge, this paper is the first systematic review of Mamba architectures in remote sensing. Our work provides a structured foundation for advancing research in remote sensing systems through SSM-based methods. We curate an open-source repository (https://github.com/BaoBao0926/Awesome-Mamba-in-Remote-Sensing) to foster community-driven advancements.

==> Sec/record.tex <==




\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.32\textwidth} % 第一列
        \centering
        \includegraphics[width=\textwidth]{picture/SSMFormula/ContextSSMpng.png} % 替换为你的图片路径
        \caption{The core idea of the Context-SSM is to allow SSM to model long-range dependencies while taking local context into consideration \cite{62-Mamba-MOC, 35-AFA-Mamba}.}
        \label{fig:contextSSM}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth} % 第二列
        \centering
        \includegraphics[width=\textwidth]{picture/SSMFormula/crossSSM.png} % 替换为你的图片路径
        \caption{
        The core idea of the Cross-SSM is to naturally interact two modality features in SSM formula \cite{5-S2CrossMamba, 84-COMO}.}
        \label{fig:crossSSM}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth} % 第三列
        \centering
        \begin{subfigure*}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{picture/SSMFormula/discretization.png} 
            \caption{Using higher-order discretization method, RK2 \cite{RK2}, to improve the continuous sequence approximation \cite{112-RSVMamba}.}
            \label{fig:discretizationSSM}
        \end{subfigure*}
        \vfill
        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{picture/SSMFormula/hiddenState.png} 
            \caption{New definition of hidden state for SSM. Tree Topology SSM is customized for tree scan pattern \cite{68-TTMGNet}.}
            \label{fig:HiddenSSM}
        \end{subfigure}
    \end{minipage}
    % \caption{full}
\end{figure*}





\begin{table}[]
% \rightarrow  → 左  
% \downarrow   ↓ 右 
% \nwarrow ↖ （North-West，左上）
% \swarrow ↙ （South-West，左下） 
% \nearrow ↗ （North-East，右上） 
% \searrow ↘ （South-East，右下）
\resizebox{\linewidth}{!}{ 
\begin{tabular}{l|ccccc|l}
\hline
\multirow{2}{*}{Scan Name} & \multicolumn{5}{c|}{Scan Strategy} & \multirow{2}{*}{Papers} \\ \cline{2-6}
                           & \multicolumn{1}{c|}{Bran}          & Preprocessing           & Sampling & Direction & Pattern &            \\ \hline
% 1
Vallian Scan            & \multicolumn{1}{c|}{-} & -  & -        & \nwarrow(\rightarrow) & Z   &  \cite{5-S2CrossMamba,6-CDMamba,8-IMDCD,13-Samba,15-CMS2I-Mamba,20-SC-Mamba,27-HLMamba,33-SpectralMamba,39-MSTFNet,42-PyramidMamba,43-MorpMamba,45-DualMamba,49-SS-Mamba,52-SSRFN,53-ConvMambaSR,61-WaveMamba,62-Mamba-MOC,63-GraphMamba,73-HTD-Mamba,74-SITSMamba,75-ES-HS-FPN,78-CSMN,89-HSIRMamba,101-MambaHSI,103-SCMamba }    \\ \hline
% 2
Window Scan             & \multicolumn{1}{c|}{-} & -  & Window & \nwarrow(\rightarrow) & Z     &  \cite{82-HDMba}                       \\ \hline
% 3
Hibert Scan             & \multicolumn{1}{c|}{-} & - & -       & \swarrow(\downarrow)  & Hibert&  \cite{95-LDMNet}                       \\ \hline
% 4
Bi-Scan                & \multicolumn{1}{c|}{-}  & - & -  & \nwarrow\searrow(\rightarrow)& Z   &   \cite{11-S2CrossMamba, 28-FusionMamba,31-HyperMamba,47-SegMamba-OS,48-RSCaMa,64-S2Mamba,67-DTAM,76-MamTrans,85-YOLO-Mamba,93-HSIMamba,107-MLMamba,113-TrackingMamba }                      \\ \hline
% 5
\begin{tabular}[c]{@{}l@{}}Spectral \\ Bi-Scan-1\end{tabular} & \multicolumn{1}{c|}{-} & \multicolumn{1}{l}{IB: SaT-1} & -  & \nwarrow\searrow(\rightarrow) & Z & \cite{29-MSFMamba,45-DualMamba,46-LE-Mamba } \\ \hline
% 6
\begin{tabular}[c]{@{}l@{}}Spectral \\ Bi-Scan-2\end{tabular} & \multicolumn{1}{c|}{-} & \multicolumn{1}{l}{IB: SaT-2} & -   & \nwarrow\searrow(\rightarrow)& Z & \cite{38-MambaLG} \\ \hline
% 7
Bi Scan-Hor\&Ver   & \multicolumn{1}{c|}{-} & -   & -  & \nwarrow(\rightarrow\downarrow)& Z    &  \cite{35-AFA-Mamba} \\ \hline
% 8
\begin{tabular}[c]{@{}l@{}}Bi-Local \\ Scan-Hor\&Ver\end{tabular} & \multicolumn{1}{c|}{-} & - & - & \nwarrow(\rightarrow\downarrow) & Local &   \cite{26-CVMH-UNet}\\ \hline
% 9
GSRM Bi-scan    & \multicolumn{1}{c|}{-} & \multicolumn{1}{l}{IB: GSRM} & - & \nwarrow\searrow(\rightarrow) & Z &  \cite{111-HSRMamba} \\ \hline
% 10
SS2D scan        & \multicolumn{1}{c|}{-} & -      & -      & \nwarrow\searrow(\rightarrow\downarrow)       & Z  & \begin{tabular}[c]{@{}l@{}@{}}\cite{2-RS3Mamba,3-RTMamba,4-FreMamba,7-RSDehamba,11-S2CrossMamba,12-DMM,14-ChangeMamba,15-CMS2I-Mamba,16-DC-Mamba,17-RSMamba,18-UNetMamba,19-Mamba-CR,22-Mamba-Diffusion,23-MFMamba,25-CM-UNet,28-FusionMamba,30-Res-Mamba,31-HyperMamba,32-RemoteDet-Mamba,34-MambaFormer,37-HSDet-Mamba,40-PPMamba, 41-MF-VMamba,44-UVMSR,47-SegMamba-OS}\\ \cite{49-SS-Mamba,53-ConvMambaSR,60-SSUM,69-EGCM-UNet,72-RFCC} \\ \cite{75-ES-HS-FPN,80-FMambaIR,83-MTIE-Net,84-COMO,86-Prompt-Mamba,87-Mamba-UAV-SegNet,91-SDMSPan,97-MGMF,99-MiM-ISTD,102-LCCDMamba,104-HMCNet,105-Mamba-MDRNet,108-SatMamba,112-RSVMamba} \end{tabular} \\ \hline



% 11
\begin{tabular}[c]{@{}l@{}}S-Shape \\ SS2D scan\&Ver\end{tabular}     & \multicolumn{1}{c|}{-} & -      & -      & \nwarrow\searrow(\rightarrow\downarrow)       & S  &   \cite{85-YOLO-Mamba,96-MaDiNet} \\ \hline
% 12
Local SS2D scan & \multicolumn{1}{c|}{-} & -      & -      & \nwarrow\searrow(\rightarrow\downarrow)  & Local   & \cite{46-LE-Mamba}   \\ \hline
% 13
LP-SS2D scan & \multicolumn{1}{c|}{-}  & \multicolumn{1}{l}{IB: LP} & -  & \nwarrow\searrow(\rightarrow\downarrow) & Z & \cite{81-ColorMamba}\\ \hline
% 14
SE-VSS scan    & \multicolumn{1}{c|}{-}  & \multicolumn{1}{l}{IB: SE}  & - & \nwarrow\searrow(\rightarrow\downarrow) & Z &  \cite{88-VMambaSCI}            \\ \hline
% 15
\begin{tabular}[c]{@{}l@{}}Center Pixel \\ Scan\end{tabular} & \multicolumn{1}{c|}{-} & -  & -  & \begin{tabular}[c]{@{}c@{}}Center Token\\ Clockwise\end{tabular} & Helical  & \cite{59-STMamba} \\ \hline
% 16
\begin{tabular}[c]{@{}l@{}}Tree Topology \\ Scan\end{tabular}& \multicolumn{1}{c|}{-} & -  & -  & \nwarrow(\rightarrow) & Tree &    \cite{68-TTMGNet}                 \\ \hline
% 17
3D Scan & \multicolumn{1}{c|}{-} & -  & -  & \begin{tabular}[c]{@{}c@{}}12 Directions\\ Fig.?\end{tabular} & \begin{tabular}[c]{@{}c@{}}3D \\ S\end{tabular}  & \cite{79-SSUMamba}   \\ \hline
% 18
\multirow{2}{*}{Omni Scan-1} & 
    \multicolumn{1}{c|}{\multirow{2}{*}{Para}} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{\nwarrow\searrow(\rightarrow\downarrow)} & Z  & \multirow{2}{*}{}    \\
  & \multicolumn{1}{c|}{}   &  & &   & Diagonal   &        \cite{1-RS-Mamba,21-UV-Mamba,56-PPMamba }                 \\ \hline
% 19
Omni Scan-2  & \multicolumn{1}{c|}{-} & -  & -  & \nwarrow\nearrow\searrow\swarrow(\rightarrow\downarrow)  & S  &  \cite{36-MiM}                       \\ \hline
% 20
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Random Scan \&\\ Bi-Scan\end{tabular}} & 
    \multicolumn{1}{c|}{\multirow{2}{*}{Para}} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \nwarrow\searrow(\rightarrow)& Z & \multirow{2}{*}{}       \\
    & \multicolumn{1}{c|}{}  &         &   & \nwarrow(\rightarrow)  & Random    &   \cite{9-RSMamba,15-CMS2I-Mamba,109-UrbanSSF }                      \\ \hline
% 21
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Spectral Random \\ Scan \& Bi-Scan\end{tabular}}  
    & \multicolumn{1}{c|}{\multirow{2}{*}{Para}} & -  & -  & \nwarrow\searrow(\rightarrow) & Z  & \\
    & \multicolumn{1}{c|}{}  & \multicolumn{1}{l}{IB: SaT-1}  & -   & \nwarrow(\rightarrow) & Random &   \cite{15-CMS2I-Mamba} \\ \hline
% 22
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Random Scan\\ \&SS2D Scan\end{tabular}} 
& \multicolumn{1}{c|}{\multirow{2}{*}{Para}} & \multirow{2}{*}{-}  & \multirow{2}{*}{-} & \nwarrow\searrow(\rightarrow\downarrow) & Z &    \\
& \multicolumn{1}{c|}{}                      &                     &                    & \nwarrow(\rightarrow)               & Random&  \cite{92-MambaDS}  \\ \hline
% 23
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Multi-Router \\ Scan-1\end{tabular}} 
& \multicolumn{1}{c|}{\multirow{2}{*}{Para}} & \multirow{2}{*}{-}  & \multirow{2}{*}{-} & \multirow{2}{*}{\nwarrow(\rightarrow\downarrow)} & Z & \multirow{2}{*}{}       \\
& \multicolumn{1}{c|}{}                      &                     &                   &         & S         &   \cite{24-LightMamba}   \\ \hline
% 24
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Multi-Router \\ Scan-2\end{tabular}}  & 
    \multicolumn{1}{c|}{\multirow{2}{*}{Para}} & \multirow{3}{*}{-} & \multirow{3}{*}{-}      & \multirow{3}{*}{\nwarrow(\rightarrow)} & Z    & \multirow{3}{*}{}       \\
    & \multicolumn{1}{c|}{}                    &                    &                         &                                        & S    &                         \\
    & \multicolumn{1}{c|}{}                    &                    &                         &       & Diagonal  & \cite{106-Weaba}       \\ \hline
% 25
\multirow{2}{*}{Cross Scan} 
    & \multicolumn{1}{c|}{\multirow{2}{*}{Para}} & \multirow{2}{*}{-} & \multirow{2}{*}{-}& \multirow{2}{*}{\nwarrow\searrow(\rightarrow)} & Z  & \multirow{2}{*}{}       \\
    & \multicolumn{1}{c|}{}                      &                    &                   &    & Diagonal                     &    \cite{26-CVMH-UNet}\\ \hline
% 26
\multirow{2}{*}{Efficient Scan}               
    & \multicolumn{1}{c|}{\multirow{2}{*}{Para}} & \multirow{2}{*}{-} & \multirow{2}{*}{Atrous} & \nwarrow(\rightarrow) & Z & \multirow{2}{*}{}       \\
    & \multicolumn{1}{c|}{}                      &                    &                         & \nwarrow(\downarrow)  & Z &   \cite{94-HRMamba-YOLO}\\ \hline
% 27
\multirow{2}{*}{Bi Scan-Seq} 
    & \multicolumn{1}{c|}{\multirow{2}{*}{Seq}}  & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \nwarrow(\rightarrow) & Z  & \multirow{2}{*}{}       \\
    & \multicolumn{1}{c|}{}                      &                    &                    & \searrow(\rightarrow) & Z  &    \cite{70-TransMamba} \\ \hline
% 28
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Bi-Continuous \\ Scan-Seq\end{tabular}}          
    & \multicolumn{1}{c|}{\multirow{2}{*}{Seq}}  & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \nwarrow\swarrow(\rightarrow\downarrow) & Z  & \multirow{2}{*}{}       \\
    & \multicolumn{1}{c|}{}   &  &   & \nearrow\searrow(\rightarrow\downarrow) & S  &  \cite{58-HSIDMamba}   \\ \hline
% 29
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Local\&Global \\ Spatial Scan-Seq\end{tabular}} 
    & \multicolumn{1}{c|}{\multirow{2}{*}{Seq}}  & \multirow{2}{*}{-} & Window & \nwarrow(\rightarrow) & S  &                         \\
    & \multicolumn{1}{c|}{}     &       & -      & \nwarrow(\rightarrow) & S  & \cite{38-MambaLG}   \\ \hline
% 30
\multirow{2}{*}{3DSS Scan}                    
    & \multicolumn{1}{c|}{\multirow{2}{*}{Seq}}  & -                  & -   & \nwarrow\searrow(\rightarrow)  & S   &                         \\
    & \multicolumn{1}{c|}{}        & \multicolumn{1}{l}{IB: SaT-1}    & -   & \nwarrow\searrow(\rightarrow)  & S   &  \cite{55-3DSS-Mamba} \\ \hline
% 31
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Multi-Scale \\ Spatial Scan\end{tabular}} 
    & \multicolumn{1}{c|}{\multirow{2}{*}{Seq}}  & \multicolumn{1}{l}{IB: $\text{Conv}_{s=1}$} & - & \nwarrow(\rightarrow\downarrow) & S  &   \\
    & \multicolumn{1}{c|}{}   & \multicolumn{1}{l}{IB: $\text{Conv}_{s=2}$} & - & \nwarrow(\rightarrow\downarrow) & S  & \cite{29-MSFMamba} \\ \hline
% 32
\multirow{2}{*}{Group Scan}                   
    & \multicolumn{1}{c|}{\multirow{2}{*}{Seq}}  & \multicolumn{1}{l}{IB: CG}  & -   & \nwarrow(\rightarrow)  & S   &                         \\
    & \multicolumn{1}{c|}{}          & \multicolumn{1}{l}{IB: SaT-1+CG}        & -   & \nwarrow(\rightarrow)  & S   &  \cite{51-IGroupSS-Mamba} \\ \hline
% 33
\begin{tabular}[c]{@{}l@{}}Nested Shift \\ Scan\end{tabular}  & \multicolumn{1}{c|}{-} & \multicolumn{1}{l}{BB: SSM}             
    & -   & \nwarrow\searrow(\rightarrow\downarrow) & \begin{tabular}[c]{@{}c@{}}Nested \\ S-Shape\end{tabular} & \cite{90-MaIR} \\ \hline
% 34
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Locally Apaptive\\ Scan\end{tabular}}  
    & \multicolumn{1}{c|}{\multirow{2}{*}{-}}   & \multicolumn{1}{l}{IB: ABRM}  & \multirow{2}{*}{-} & \multirow{2}{*}{\nwarrow(\rightarrow)}  & \multirow{2}{*}{S} &  \\
    & \multicolumn{1}{c|}{}     & \multicolumn{1}{l}{BB: WSM}       &            &              &        &   \cite{110-CD-Lamba} \\ \hline
\end{tabular}
}
\end{table}


\begin{table*}[]
\renewcommand{\arraystretch}{1.38} % 调整行距
\resizebox{\linewidth}{!}{ 
\begin{tabular}{cccl}
\hline
\multicolumn{4}{l}{\cellcolor[HTML]{C0C0C0}\textbf{Section III.1 Interation with CNN and Transformer}}   \\ \hline

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{Seq}  
        & \begin{tabular}[c]{@{}l@{}}{\cite{11-S2CrossMamba, 16-DC-Mamba, 19-Mamba-CR, 30-Res-Mamba, 53-ConvMambaSR, 92-MambaDS, 44-UVMSR, 27-HLMamba, 34-MambaFormer, 40-PPMamba, 45-DualMamba, 71-LS2SM-MHMambaOut}[}29{]}, {[}34{]}, {[}37{]}, {[}49{]}, {[}69{]}, {[}72{]}, {[}76{]}, {[}78{]}, {[}80{]}, {[}82{]},  {[}109{]}, {[}135{]}.  \\ 
        \cite{46-LE-Mamba, 78-CSMN, 38-MambaLG, 56-PPMamba, 102-LCCDMamba, 83-MTIE-Net} {[}42{]}, {[}59{]}, {[}60{]}, {[}87{]}, {[}93{]}, {[}105{]}, \cite{69-EGCM-UNet} EFCM-Unet{[}84{]}  \\ 
        \cite{46-LE-Mamba, 38-MambaLG, 56-PPMamba, 78-CSMN, 92-MambaDS, 93-HSIMamba, 111-HSRMamba} {[}56{]}, {[}59{]}, {[}60{]}, {[}62{]}, {[}105{]},{[}109{]}, \cite{63-GraphMamba, 21-UV-Mamba, 52-SSRFN} Graph-Mamba,UV-Mamba,SSRFN\end{tabular}                                    \\ \cline{3-4} 
        
\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{\multirow{-2}{*}{Unit}} & \multicolumn{1}{c|}{Para} 
        & \cite{21-UV-Mamba, 8-IMDCD, 23-MFMamba, 40-PPMamba, 41-MF-VMamba, 99-MiM-ISTD, 102-LCCDMamba} {[}26{]}, {[}74{]}, {[}80{]}, {[}81{]}, {[}92{]}, {[}93{]}, {[}104{]} \\ \cline{2-4} 
        
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{Seq}  
        & \begin{tabular}[c]{@{}l@{}}{ \cite{2-RS3Mamba, 8-IMDCD, 23-MFMamba, 40-PPMamba, 41-MF-VMamba, 99-MiM-ISTD, 102-LCCDMamba} [}26{]}, {[}65{]}, {[}74{]}, {[}80{]}, {[}81{]}, {[}92{]}, {[}93{]}, \cite{25-CM-UNet, 42-PyramidMamba, 72-RFCC, 96-MaDiNet}{[}32{]}, {[}75{]}, {[}85{]}, {[}97{]}.   \\ 
          \cite{3-RTMamba, 5-S2CrossMamba, 20-SC-Mamba, 33-SpectralMamba, 54-DBMamba, 59-STMamba} {[}16{]}, {[}28{]}, {[}30{]}, {[}66{]}, {[}101{]}, {[}138{]}, \cite{25-CM-UNet, 42-PyramidMamba, 72-RFCC, 96-MaDiNet}{[}32{]}, {[}75{]}, {[}85{]}, {[}97{]}\end{tabular}     \\ \cline{3-4} 
\multicolumn{1}{c|}{\multirow{-4}{*}{CNN}}     & \multicolumn{1}{c|}{\multirow{-2}{*}{Arch}} & \multicolumn{1}{c|}{Para} 
        & \cite{53-ConvMambaSR, 65-ConMamba, 86-Prompt-Mamba, 89-HSIRMamba, 103-SCMamba, 104-HMCNet, 106-Weaba} {[}37{]},{[}43{]}, {[}45{]}, {[}88{]}, {[}94{]}, {[}111{]}, {[}133{]}. \cite{2-RS3Mamba} S3Mamba {[}65{]} and \cite{81-ColorMamba} ColorMamba {[}98{]} \\ \hline
\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Seq}  
        &  \cite{17-RSMamba, 19-Mamba-CR, 20-SC-Mamba, 43-MorpMamba, 77-MHSSMamba, 91-SDMSPan} {[}28{]}, {[}33{]}, {[}70{]}, {[}72{]}, {[}90{]}, {[}139{]}, {[}90{]}  \\ \cline{3-4} 
\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{\multirow{-2}{*}{Unit}} & \multicolumn{1}{c|}{Para} 
        & \cite{23-MFMamba} MFMamba {[}74{]} and \cite{34-MambaFormer} MambaFormerSR {[}78{]}, \cite{70-TransMamba}  TransMamba {[}113{]} \\ \cline{2-4} 
\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{Seq}  
        & \begin{tabular}[c]{@{}l@{}} \cite{39-MSTFNet} MSTFNet {[}31{]}, \cite{42-PyramidMamba} pyramidMamba {[}32{]}, \cite{18-UNetMamba} UNetMamba {[}71{]}, and \cite{96-MaDiNet} MaDiNet   \\ {[}97{]}, \cite{48-RSCaMa} RSCaMa {[}51{]} and \cite{105-Mamba-MDRNet} Mamba-MDRNet {[}95{]}\end{tabular}  \\ \cline{3-4} 
        
\multicolumn{1}{c|}{\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Trans-\\ former\end{tabular}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{Arch}} 
    & \multicolumn{1}{c|}{Para} & \cite{76-MamTrans} MamTran     \\ \hline
\multicolumn{3}{c|}{Mamba as Module}                                                                                                                                     & {[}17{]},{[}22{]}, \cite{6-CDMamba, 11-S2CrossMamba, 12-DMM, 32-RemoteDet-Mamba, 47-SegMamba-OS, 84-COMO, 110-CD-Lamba} {[}25{]}, {[}49{]}, {[}63{]}, {[}77{]}, {[}100{]}, \cite{37-HSDet-Mamba} HSDet-Mamba {[}79{]} and \cite{87-Mamba-UAV-SegNet} Mamba-UAV-SegNet {[}89{]} \cite{75-ES-HS-FPN} ES-HS-FPN {[}41{]}  \\ \hline



\multicolumn{4}{l}{\cellcolor[HTML]{C0C0C0}\textbf{Section III.2 Substitution}}  \\ \hline
\multicolumn{3}{c|}{U-Net}      & \cite{2-RS3Mamba, 7-RSDehamba, 11-S2CrossMamba, 14-ChangeMamba,16-DC-Mamba, 17-RSMamba, 18-UNetMamba, 19-Mamba-CR, 20-SC-Mamba, 21-UV-Mamba, 23-MFMamba, 24-LightMamba, 25-CM-UNet, 26-CVMH-UNet, 40-PPMamba, 41-MF-VMamba, 44-UVMSR, 56-PPMamba, 66-DHM, 69-EGCM-UNet, 70-TransMamba, 72-RFCC, 79-SSUMamba, 80-FMambaIR, 81-ColorMamba, 83-MTIE-Net, 98-LGMamba, 99-MiM-ISTD, 102-LCCDMamba, 104-HMCNet, 106-Weaba, 109-UrbanSSF }                            \\ \hline
\multicolumn{3}{c|}{YOLO}       & \cite{37-HSDet-Mamba, 75-ES-HS-FPN, 85-YOLO-Mamba, 94-HRMamba-YOLO} \\ \hline
\multicolumn{3}{c|}{Diffusion}  & \cite{8-IMDCD, 96-MaDiNet}                                          \\ \hline
\multicolumn{3}{c|}{CLIP}       &  \cite{48-RSCaMa}                                                   \\ \hline


\multicolumn{4}{l}{\cellcolor[HTML]{C0C0C0}\textbf{Section III.3 learning paradigm}}   \\ \hline
\multicolumn{3}{c|}{unsurpervised}      &  \cite{72-RFCC}                       \\ \hline
\multicolumn{3}{c|}{self-learning}      &  \cite{73-HTD-Mamba, 108-SatMamba}    \\ \hline
\multicolumn{3}{c|}{week-surpervised}   &  \cite{86-Prompt-Mamba}               \\ \hline


\multicolumn{4}{l}{\cellcolor[HTML]{C0C0C0}\textbf{Section III.4 Frequency domain}}  \\ \hline
\multicolumn{3}{c|}{Fourier}            &  \cite{4-FreMamba, 26-CVMH-UNet, 34-MambaFormer, 70-TransMamba, 78-CSMN, 80-FMambaIR, 87-Mamba-UAV-SegNet } \\ \hline
\multicolumn{3}{c|}{wavelet}            &  \cite{61-WaveMamba} \\ \hline

\end{tabular}
}
\caption{aaaa}
\end{table*}


\section{Introduction}
% introduction to CNN/transofmrer
Recent advances in remote sensing have increasingly leveraged deep learning-based methods to extract meaningful features from the data \cite{survey5, survey_remote}. Conventional approaches, including Convolutional Neural Networks (CNNs) and Vision Transformers (ViTs), have achieved significant success in remote sensing. CNNs have advantages of linear computational complexity and versatile modeling ability \cite{1,2,3}, but are limited to its local receptive field. ViTs utilize self-attention mechanism \cite{Transformer, ViT} to achieve global modeling, but is limited to its quadratic computational complexity, which is unacceptable for some high-resolution data in remote sensing. Although CNNs and ViTs have such limitations, computer vision domain, including remote sensing domain, has been dominated by CNNs and ViTs for long time. Therefore, naturally, some researchers want to find a method that can achieve global modeling with only linear computation complexity.



% SSM->S4->S6
Recently, some state space model (SSM)-based methods have generated great attention due to their linear computation complexity and global modeling. SSM is a classic theory that is widely adopted in various disciplines, such as Markov decision process in reinforcement learning \cite{10}, dynamic causal modeling in computational neuroscience \cite{11} and Kalman filters in controls \cite{12}. The core idea is mapping input into the intermediate hidden state that can be regarded as summary of previous information, and then predict the next output based on the hidden state and current input. Recently, some work has tried to incorporate SSM into deep learning framework \cite{s4, HIPPO, HIPPO2, H3, 14, 15, 16, 17, ssm, mamba, Mambav2}. At very beginning, SSM-based methods are not widely used due to low computation burden and memory requirement \cite{survey5}. However, structure SSM (S4) preliminarily addresses this issue by parameterizing the state matrices $\textbf{A}$ \cite{s4}. After that, Selective SSM (S6) \cite{mamba} introduces a selective mechanism that can regress time step size \( \boldsymbol{\Delta} \) to selectively propagate or forget information stored in the hidden states. Mamba \cite{mamba} incorporates S6 block into a simplified gated architecture, thus achieving the state-of-the-art (SOTA) performance and becoming a renowned architecture.

% NLP->CV->remote sensing
Originally designed for Natural Language Processing (NLP), some researchers quickly adapt Mamba into Computer Vision (CV) field. Like the operations of Vision Transformer (ViT) \cite{ViT}, two foundational vision Mamba backbone works, Vision Mamba (Vim) \cite{VisionMamba} and Visual Mamba (VMamba) \cite{VMamba}, embed the image into several patches, and then scan (transform) these patches from several directions into several 1D sequences, which can be input into Mamba blocks. Then, the subsequent Mamba-based models continue to improve performance from various perspective, thus leading to that Mamba-based model achieve SOTA performance in each CV sub-fields.

Remote sensing, as an important sub-field in CV, is inevitably explored by many researchers who try to utilize Mamba-based model to solve the potential problems of CNNs and Transformer. Remote sensing images usually have these challenges: 1) Remote sensing images are full of spatial information, which causes the local receptive field of CNNs to not model the whole image very well; 2) Remote sensing images often have very high resolution or very large-size images, which can lead to unacceptable computational complexity in Transformer based networks. Because of this, Mamba-based method can solve these two drawbacks perfectly in theory. There have been a lot of works that have basically validated Mamba-based models in remote sensing. In general, they have reached SOTA performance. 

Among so many work in remote sensing, we found that there was a lack of a proper survey paper to categorize existing methods and help researchers quickly understand how Mamba-based methods in remote sensing work. Therefore, this paper summarizes totally 113 papers in the field of remote sensing, and make a series of classifications to help researchers quickly understand the status of Mamba-based model. Our contributions and structures are summarized as follows:

\begin{enumerate}
    \item \textbf{Preliminary Knowledge} (Section \ref{sec:PreKnow}): We provides an introduction to the SSM, Mamba \cite{mamba}, and Mamba-2 \cite{Mambav2}.
    \item \textbf{Vision Mamba Backbone} (Section \ref{sec:vision_mamba}): We provides a brief introduction for vision Mamba backbone network, in order to help understand the basic concepts and innovations.
    \item \textbf{Micro-Architecture Advancement} (Section \ref{sec:micro}): We provides detailed innovations from the perspective of micro-architecture, including SSM formula improvement, scan strategy improvement, and multi-modality and bi-temporal fusion improvement.
    \item \textbf{Macro-Architecture Advancement} (Section \ref{sec:macro}): We provides detailed innovation from the perspective of macro-architecture, including hybrid architecture with CNNs and transformers, substitution of existing frameworks, learning paradigms and frequency domain operations.
    \item \textbf{Downstream Tasks} (Section \ref{sec:downstramtask}): We build up benchmark tables for classification, segmentation, change detection, object detection, super-resolution and image restoration tasks. In addition, we briefly talked about the works focusing on uncommon tasks.
    \item \textbf{Challenges and Future Directions} (Section \ref{sec:direction}): We examine the challenge existing in the remote sensing, and point out several promising future directions that may potentially improve Mamba-based model.
    \item \textbf{Conclusion} (Section \ref{sec:conclusion}): We briefly summarize the whole paper.
\end{enumerate}








\section{Vision Mamba Backbone}

In this section, we review some representative visual Mamba backbone network to clarify the fundamental principles and innovations of applying Mamba to CV. We more focus the innovations related with Mamba block.


Since the emergence of the two foundation articles Vim and VMamba, a large number of subsequent backbone network articles have appeared. These paper focuses several aspects, including novel scanning strategies \muyi{Mamba-ND, LocalVMamba, PlainMamba}, following the previous work in CNN/Transformer \muyi{}, 

\subsection{Novel Scanning Strategies}
Mamba-ND \muyi{Mamba-nd} is the first paper to explore a generalized framework for modeling multi-dimensional data, such as video data. Mamba-ND design to scan along the $Height$, $Width$ and $Time$ dimensions with sequential alternation in block level.
LocalMamba \cite{LocalMamba} introduces local scan strategy to address the discontinuity of the original scan strategy. It proposes local scan strategy that first scan the patches within a local window and then move to the next window, which can enhance Mamba block's understanding of local context features, as shown in Fig. \ref{fig:ScanStrategy}.4D. In addition, inspired by DARTS \muyi{DARTS: Differentiable architecture search}, LocalMamba utilize a learnable factor to decide scan strategies in four pathways. 
Similarly, PlainMamba \cite{plainmamba} introduces continuous 2D scanning method that scans the whole image continuously, as shown in Fig. \ref{fig:ScanStrategy}.4B. This scan strategy ensures the continuity of transforming 2D image into sequence, addressing issue of discontinuity in Vim \cite{VisionMamba} and VMamba \cite{VMamba}. Additionally PlainMamba is a non-hierarchy architecture without any special tokens, which also show a competitive performance.
MS-VMamba \muyi{MS-VMamba} introduces Multi-Scale 2D-Selective Scan (MS2D), which perform SSMs on original features and down-sampled features. This methods can maintain fine-grained feature while mitigating the forgetting issue.
FractalMamba \muyi{fractalMamba} introduce a novel scanning strategy, inspired by fractral theory \muyi{fractral theroy}. It uses Hilbert curve as scanning pattern with a shifted mechanism, which can follow the complex contours and structures within an image and preserve the continuity.



\subsection{Following the CNN/Transformer's work}
Following the framework of MLP-Mixer \muyi{MLP-mixer}, MambaMixer \muyi{MambaMixer} integrates Mamba for block token and channel mixing, enabling data-dependent selection and fusion of information across these dimensions. In addition, MambaMixer proposes a weighted averaging mechanism, allowing layers to access the previous layer feature, similar to the DenseNet \muyi{DenseNet} and DenseFormer \muyi{DenseFormer}.
Following the framework of \muyi{Vision transformers need registers}, MambaR \muyi{MambaR} evenly insert register tokens into the input sequences and recycle registers for final decision predictions, which can helps model to focus on more semantic regions.
Similar to the GPT family \muyi{ChatGPT, GPT-4, iGPT}, ARM \muyi{ARM} utilizes the autoregressive modeling self-supervised framework that enhances Mamba's visual capabilities by leveraging to predict clustered image patches in a unidirectional sequence, which achieves accelerated training speeds and scalable performance and establishes a foundation for large-scale vision applications with state-space models.


% don't know
SiMBA \muyi{SiMBA} introduces a novel architecture that leverages Mamba for sequence modeling, addressing its instability when scaled to large networks on vision datasets by incorporating a new channel modeling technique called EinFFT. By combining Mamba with EinFFT's frequency-domain channel mixing, SiMBA achieves competitive results on CV and time-series benchmarks.






% first work
Vim-F \muyi{Vim-F} is the first paper that introduces frequency domain information to achieve a better global receptive field during the scanning process.

% hybrid model
MambaVision \muyi{MambaVision} redesigns the Mamba architecture and integrates CNNs and ViT block into the macro-architecture, aiming at enhancing modeling capability.
% one method
In order to address the instability and inefficiency of large model sizes, GroupMamba \muyi{GroupMamba} introduce Modulated Group Mamba Layer that divides the input into four groups in channel dimensions and applies SSMs independently to each groups with a channel-based attention mechanism and a distillation-based training objective.
% SSM formula
VSSD \muyi{VSSD} extend SSD in Mamba-2 \cite{Mambav2} into a non-causal visual state space duality (VSSD) by discarding the magnitude of interactions between the hidden state and tokens, which is designed for non-causal data, such as image data.
% 
ShuffleMamba \muyi{16ShuffleMamba} introduces Stochastic Layer-Wise Shuffle (SLWS), a training regularization technique designed to mitigate overfitting and enhance the scalability of Vision Mamba models by randomly shuffling token sequences during training to improve positional transformation invariance and overall model performance.
% 
StableMamba \muyi{17}, a Mamba-Attention interleaved architecture that addresses the scalability and robustness challenges of large-scale State-Space Models (SSMs) for image and video recognition, enabling efficient scaling to over 100M parameters without requiring knowledge distillation while improving performance and robustness to common image corruptions.
% 
SparX-Mamba \muyi{18} introduces a efficient sparse cross-layer feature aggregation method specifically designed for SSMs.
% 
\muyi{20} introduces a token pruning method specifically designed for Mamba-based model.









\section{Vision Mamba Backbones} \label{sec:vision_mamba}

This section some reviews vision Mamba backbone networks. We recommend to see other survey \cite{survey1, surveyon2, survey6, survey5} that can provide more detailed discussion of vision mamba backbone. We first introduce two seminal works using Mamba in the CV field to present the basic ideas, and then introduce subsequent work.

Vision Mamba (Vim) \cite{VisionMamba} is the first paper to apply Mamba in CV. Following the framework of ViT \cite{ViT}, Vim first embeds the images into 2D patches, which are then vectorized 2D patches by CNNs and are added with position embeddings to retain spatial information, which is the common practice for future works. Additionally, Vim append a class token in order to conduct classification. To address the inherent causality issue of SSMs, Vim proposes the bi-directional scan that first flatten the 2D patches and then incorporates a backward pathway that scan the entire 1D picture patch sequence from back to front along with the forward pathway. The overall structure of Vim is composed of identical such Vim blocks.

Visual Mamba (VMamba) \cite{VMamba} focuses on the two challenges: 1) 1D CNN before SSMs is not suitable for 2D images 2) the inherent casual property of SSMs that transforms 2D patches into 1D sequences. In order to address these two challenges, VMamba proposes Cross-Scan Module (CSM). First, CSM replaces 1D CNNs with 2D Depth-Wise convolutional layers (DWConv) to extract contextual information of the images, which becomes a common practice in the later work. Second, CSM uses 2D-Selective-Scan (SS2D) that scans the whole image from four directions, the top-left patch and the bottom-right patch vertically and horizontally, and finally add the 1D sequences of four pathway together. SS2D addresses the gap between the ordered nature of selective SSMs to some extent from the perspective of scanning from different directions.

Considering a fundamental challenge in adapting SSMs to vision tasks lies in effectively transforming 2D spatial relationships into sequential representations, a lot of work has focused on modifying scan strategies to increase the model's understanding of non-causal 2D data.
Based on Vim and VMamba, \textbf{Mamba-ND} \cite{MambaND} generalizes the scan strategy to 3D data with block-level alternation of directions along height/width/time axes. 
After that, some work focus on scan patterns (discussed in Section \ref{sec:scan pattern}). 
\textbf{LocalVMamba} \cite{LocalMamba} combines local window-based scanning (Fig.~\ref{fig:ScanStrategy}.4D) with learnable pathway weights using DARTS-inspired \cite{DARTS} architecture search.
\textbf{PlainMamba} \cite{plainmamba} implements non-hierarchical architecture with continuous 2D scan (Fig.~\ref{fig:ScanStrategy}.4B) to address the issue of discontinuity.
\textbf{FractalMamba \cite{FractralMamba}} employs Hilbert curve patterns (Fig.~\ref{fig:ScanStrategy}.4E) with shift mechanisms to allow model to focus on natural image contours.
Then, some papers use some preprocessing methods (discussed in Section \ref{sec:mulplePre}) to enhance the performance of SSMs.
\textbf{MS-VMamba} \cite{MSVMamba} applies two SSMs on the original and down-sampled features independently, which can maintain fine-grained features while mitigating the forgetting issue, as shown in Fig. \ref{fig:ScanStrategy}.1I.
\textbf{GroupMamba} \cite{GroupMamba} introduce Modulated Group Mamba Layer that divides the input into four groups in channel dimensions and applies one SSM independently to each groups with a channel-based attention mechanism and a distillation-based training objective.


Some researchers have developed Mamba-based architecture on designs that are proven effective in CNN/Transformer blocks.
\textbf{MambaMixer} \cite{MambaMixer} follows the core idea of MLP-Mixer \cite{MLP-Mixer} to combine Mamba-based token mixing with channel mxiing, and follows the design of DenseNet \cite{DenseNet} and DenseFormer \cite{DenseFormer} to allow blocks to access the previous feature.
Following \cite{TransformerR}, \textbf{MambaR} \cite{MambaR} evenly insert register tokens into the input sequences and recycle registers for final decision predictions, which can helps model to focus on more semantic regions.
\textbf{ARM} \cite{ARM} follows the GPT families \cite{iGPT, GPT4, ChatGPT}, which utilizes the autoregressive modeling self-supervised framework. This can enhance Mamba’s visual capabilities by leveraging to predict clustered image patches in a unidirectional sequence, which achieves accelerated training speeds and scalable performance and establishes a foundation for large-scale vision applications with state-space models.
Similar to EViT \cite{EViT}, \textbf{MambaPruning} \cite{MambaTokenPruning} introduces a token pruning method specifically designed for Mamba-based model. \textbf{ShuffleMamba} \cite{shuffleMamba} introduces Stochastic Layer-Wise Shuffle (SLWS), a training regularization technique designed to mitigate overfitting and enhance the scalability of Vision Mamba models by randomly shuffling token sequences during training to improve positional transformation invariance and overall model performance.

Recent advances in vision Mamba architectures have witnessed growing efforts to enhance model capabilities through specialized micro-architecture designs. 
Building upon the state-space duality (SSD) mechanism in Mamba-2 \cite{Mambav2}, \textbf{VSSD} \cite{VSSD} introduces non-causal processing by decoupling interaction magnitudes between hidden states and tokens, explicitly adapting the architecture for non-sequential visual data. This direction is further extended by 
\textbf{SparX-Mamba} \cite{SparX}, which innovates sparse cross-layer feature aggregation to optimize information flow across state-space layers. 
Meanwhile, spectral domain enhancements emerge as another promising direction - \textbf{Vim-F} \cite{Vim-F} pioneers frequency-domain feature integration during the scanning phase, effectively expanding the model's global receptive field through multi-spectral analysis. These architectural refinements demonstrate how targeted modifications to Mamba's core components can address specific challenges in visual representation learning.


The evolution of visual Mamba architectures has also seen significant breakthroughs in system-level design paradigms. 
\textbf{SiMBA} \cite{SiMBA} pioneers hybrid sequence-channel modeling through EinFFT module, effectively resolving the instability issues that plague conventional Mamba scaling in vision tasks while maintaining linear computational complexity. Parallel innovations focus on architectural hybridization - 
\textbf{StableMamba} \cite{StableMamba} establishes a robust interleaved Mamba-Attention framework that successfully scales SSMs to over 100 million parameters, demonstrating unprecedented robustness against image corruptions without resorting to knowledge distillation techniques. Complementing these directions, 
\textbf{MambaVision} \cite{MambaVision} rearchitects the fundamental Mamba block through strategic integration of CNN inductive biases and Transformer-style attention mechanisms, creating a unified architecture that synergizes the strengths of multiple visual modeling paradigms. These macroscopic innovations collectively push the boundaries of state-space models in vision, enabling more stable scaling, improved cross-domain generalization, and multi-paradigm feature fusion capabilities.




